Do high-spin high-mass X-ray binaries contribute to the population of merging binary black holes?

Gravitational-wave observations of binary black hole (BBH) systems point to black hole spin magnitudes being relatively low. These measurements appear in tension with high spin measurements for high-mass X-ray binaries (HMXBs). We use grids of MESA simulations combined with the rapid population-synthesis code COSMIC to examine the origin of these two binary populations. It has been suggested that Case-A mass transfer while both stars are on the main sequence can form high-spin BHs in HMXBs. Assuming this formation channel, we show that depending on critical mass ratios for the stability of mass transfer, 48-100% of these Case-A HMXBs merge during the common-envelope phase and up to 42% result in binaries too wide to merge within a Hubble time. Both MESA and COSMIC show that high-spin HMXBs formed through Case-A mass transfer can only form merging BBHs within a small parameter space where mass transfer can lead to enough orbital shrinkage to merge within a Hubble time. We find that only up to 11% of these Case-A HMXBs result in BBH mergers, and at most 20% of BBH mergers came from Case-A HMXBs. Therefore, it is not surprising that these two spin distributions are observed to be different.

==> cover_letter.tex <==
Dear Editor, 

We have decided to resubmit to ApJ Letters. We believe that the work presented here is timely, impactful, of broad current interest in astronomy, as well as concise, and clearly communicates an idea that can be widely understood. 

Our work concerns the spins of merging binary black holes (BBH), which is currently a highly active area of study from both binary evolution modeling and gravitational wave (GW) data analysis.  In the area of binary evolution modeling, this topic has been studied with detailed case studies (Mandel and Fragos 2020, ApJL) and population synthesis studies (Zevin and Bavera 2022).  In the area of GW data analysis, the spin distribution of BHs and its interpretation remains an open and active problem (Galaudage et al. 2021, ApJL). Additionally, with an increasing amount of GW data, population studies have been recently used to investigate discrepancies among binary populations (Fishbach and Kalogera 2022, ApJL).  Our work also concerns BH spin measurements in high-mass X-ray binaries (HMXBs; Reynolds 2021 Annual Review; Miller-Jones et al. 2021, Science), which are considered to be in tension with GW data.  We believe that our work addresses or is closely related to recent problems in these sub-fields. 

All but one of the articles cited above were published in ApJL, Science, or are an Annual Review. While not published in ApJL, the following illustrates additional current interest in modeling the spin evolution of BHs (not limited to HMXBs and merging BBHs): Qin et al 2022, Shoa and Li 2022, Antoni and Quataert 2022, Bavera et al 2022, Steinle and Kesden 2021. Although not current, the following is a list of articles published in ApJL that concern high-spin BHs in HMXBs or low-spin BHs: Batta et al. 2017, Schrøder et al. 2018, Fuller and Ma 2019. These articles show that there is interest within the community for the topics in our study and would form part of the conversation that has been on-going with ApJL. 

Our work encapsulates all three topics mentioned above: binary evolution modeling, GW data, and HMXBs.  It shows that all three can be used together to understand more than one population of binaries. On this note, our work is impactful as it is the first to offer a way to explain the spin measurements of high-spin HMXBs and BBH mergers on this level. It provides an example of understanding observed populations by analyzing different populations of binaries at once (similar methods include Bavera et al. 2022, A&A Letters). 

Measurements of BHs spins in both HMXBs and from GW mergers are expected to be better resolved in the coming years. We consider the work timely, as it is only recently (following the release of O3 results) that we have had sufficient measurements to be confident in the GW inferred spin distributions, and with the O4 run soon to begin, we can expect a rapid development of theory and population modeling (which should take into account the arguments made in our paper). 

In summary, we think the article meets the interests of ApJL readership, concisely explains a key idea that is effectively communicated in Letter format, and is timely (while building upon a conversation of previous ApJL publications), making it a good fit for the journal.

==> response_to_referee.tex <==
Referee Report Response

The authors would like to thank the referee for their helpful comments and thorough read of the manuscript. Each comment is separated with "#####" and we provide a response following the dash.


################
The paper would benefit from some further editing.
For example, what is quite confusing is that the authors use the same symbol qcrit for the critical mass ratio both for the first phase of mass transfer and for the second phase of mass transfer … This problem can be repaired by, for example, calling the critical mass ratio for the first phase of mass transfer qcrit,1 and for the second phase of mass transfer qcrit,2 (here crit,1 and crit,2 are sub-indices).

—— We have implemented your suggestion in using qcrit,MS and qcrit,BH to refer to mass transfer scenarios onto a MS star and BH. This new notation also appears in the Section 3 and Appendix. 

################
################
- On page 4, in the 11th line of the right-hand column, after the sentence ending with "respectively", add : " values similar to the latter one were also derived by Tauris et al. (2000, ApJ 530, L93), Hurley et al. (2000, MNRAS 315, 543) and Pavlovski et al. (2017, MNRAS 465, 2092).

—— This is been added on line 315. We thank the referee for pointing this similarity out.

################
################
on page 5, in the last line of the caption of Figure 2, the color "grey" is mentioned, but nowhere in the right panel of the figure there is the color grey.

—— The reference of the color “gray” has been removed from Figure 2 and is now only in the caption of Figure 3. It is left on the legend keep the two figures consistent. 

################
################
On page 6, in the 7th line of the left column, after "Belczynski et al. (2008)" add: ", due to its lower value of the critical mass ratio for HMXBs."

—— A clarifying comment similar to this has been added on L586 in Appendix A. We thank the referee for suggesting this clarification.

################
################
On page 8, in the right-hand column, at the end of the 21st line, after "forming" add "merging". And in the 28th line, before "BBHs" add "merging".

—— the word “merging” has been added here.

We have also added edited a sentence to the introduction on L133: 
"Henceforth we refer to the population of BBH systems that merge within a Hubble time as BBH, except, in cases where it can lead to confusion, we use “merging BBHs” for additional clarity."  

################
################
Page 9, 25th line of right column, after "Letter" add: "is".
(By the way, everywhere in the paper, replace "Letter" by "Paper").

—— All mentions of “Letter” have been removed.

################
################
- In the second line above section 4.2: before "BBHS" add "merging". In the 6th line of section 4.2: "occur" must be "occurs".

—— This has been addressed. Thank you for your close read. 

################
################
Final remark: I find the paper a bit long for its content. The authors should carefully go through the text once more to see where things can be written more concisely.

—— Thank you for your suggestion. Since the results across the three models are similar, the main text now only includes results for one model. Results from additional models have been moved the an appendix. We have also moved the section about alternative formation channels of high-spin HMXBs to an appendix. We think this change makes the manuscript more concise while keeping the additional information.

In appropriate locations we have included a reference to the appendix. 
For example in L163, “(Appendix A includes results for additional models).... In Appendix B we review a few alternative channels for forming a high-spin BH as the first born BH in the binary and their possible contributions to the merging BBH population.” 
